MinerU2.5: A Decoupled Vision-Language Model for Efficient High-Resolution Document Parsing

We introduce MinerU2.5, a 1.2B-parameter document parsing vision-language model that achieves state-of-the-art recognition accuracy while maintaining exceptional computational efficiency. Our approach employs a coarse-to-fine, two-stage parsing strategy that decouples global layout analysis from local content recognition. In the first stage, the model performs efficient layout analysis on downsampled images to identify structural elements, circumventing the computational overhead of processing high-resolution inputs. In the second stage, guided by the global layout, it performs targeted content recognition on native-resolution crops extracted from the original image, preserving fine-grained details in dense text, complex formulas, and tables. To support this strategy, we developed a comprehensive data engine that generates diverse, large-scale training corpora for both pretraining and fine-tuning. Ultimately, MinerU2.5 demonstrates strong document parsing ability, achieving state-of-the-art performance on multiple benchmarks, surpassing both general-purpose and domain-specific models across various recognition tasks, while maintaining significantly lower computational overhead.

==> table/task_mineru2.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabularx}{\textwidth}{@{}l l l X X X@{}}
\toprule
\textbf{Training Phase} & \textbf{Data Type} & \textbf{Data Volume} & \textbf{Data Diversity} & \textbf{Annotation Quality} & \textbf{Data Source and Annotation Method} \\ \midrule
\multirow{4}{*}{Pre-training} 
 & Layout Detection & 2.3M & General English/Chinese, exam papers, handwritten notes, PPTs, newspapers & Upper-middle & Initial annotations by MinerU1; re-annotated using multiple inferences with high temperature. Ground Truth for weak domains (e.g., newspapers) obtained via PaddleOCR + category mapping. \\
 & Text Recognition & 4.8M & Same as above & Medium & Annotated by MinerU1. \\
 & Formula Recognition & 2.2M & - & Mixed: 480k medium-quality, 650k high-quality & 480k MinerU1 annotations + 650k high-quality public datasets. \\
 & Table Recognition & 1.1M & - & Mixed: model medium, public/synthetic high & 640k model annotations + 200k public datasets + 75k synthetic data. \\ \midrule
\multirow{4}{*}{Fine-tuning} 
 & Layout Detection & 43k & Papers (Sci-Hub), textbooks, PPTs, financial reports, newspapers, exams, notes & High & Exclusively human-annotated. \\
 & Text Recognition & 900k & Sampled from Stage 1 data; 2:1 pure text vs text+formulas & Medium & Sampled via data engineering. \\
 & Formula Recognition & 441k & - & Mixed: 50k human high, 105k synthetic high, 240k public high, 48k model medium & Human-annotated (50k) + synthetic (105k) + public datasets (240k) + model (48k). \\
 & Table Recognition & 140k & - & Mixed: 25k human high, 72k model medium, 128k public high & Human-annotated (25k) + model (72k) + public datasets (128k). \\ \bottomrule
\end{tabularx}
\caption{Data sources, volumes, and annotation methods across training phases.}
\label{tab:training_data}
\end{table}


==> table/throughput_c2m.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{12pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{ccccc}
\toprule
\multicolumn{2}{c}{\textbf{Model}} & \textbf{Hardware} & \textbf{Tokens/sec} & \textbf{Pages/sec} \\
\midrule
SGLang \citep{zheng2024sglang} & \multirow{2}{*}{http server} & \multirow{3}{*}{A100 80G} & 738.66 & 0.67 \\
vLLM \citep{kwon2023efficient} & &  & 2111.88 & 1.91 \\
\cline{1-2} \cline{4-5}
vLLM & sync engine &  & 1922.92 & 1.74 \\
\cline{1-5}
\multirow{3}{*}{vLLM} & \multirow{3}{*}{\textbf{async engine}} & RTX 4090 48G & 1875.82 & 1.70 \\
% \cline{2-5}
 & & A100 80G & 2337.25 & 2.12 \\
 & & H200 141G & 4938.31 & 4.47 \\
\bottomrule
\end{tabular}
\caption{Performance Comparison of \mineru{} on Different Backends and GPUs.}
\label{tab:infer-throughput_c2m}
\end{table}

